Semantic Term "Blurring" and Stochastic "Barcoding" for Improved Unsupervised Text Classification

The abundance of text data being produced in the modern age makes it increasingly important to intuitively group, categorize, or classify text data by theme for efficient retrieval and search. Yet, the high dimensionality and imprecision of text data, or more generally language as a whole, prove to be challenging when attempting to perform unsupervised document clustering. In this thesis, we present two novel methods for improving unsupervised document clustering/classification by theme. The first is to improve document representations. We look to exploit "term neighborhoods" and "blur" semantic weight across neighboring terms. These neighborhoods are located in the semantic space afforded by "word embeddings." The second method is for cluster revision, based on what we deem as "stochastic barcoding", or "S- Barcode" patterns. Text data is inherently high dimensional, yet clustering typically takes place in a low dimensional representation space. Our method utilizes lower dimension clustering results as initial cluster configurations, and iteratively revises the configuration in the high dimensional space. We show with experimental results how both of the two methods improve the quality of document clustering. While this thesis elaborates on the two new conceptual contributions, a joint thesis by David Yan details the feature transformation and software architecture we developed for unsupervised document classification.

==> Abbreviations/listofabbr.tex <==
% \abbreviations

% % You can put here what you like, but here's an example
% %Note the use of starred section commands here to produce proper division
% %headers without bad '0.1' numbers or entries into the Table of Contents.
% %Using the {\verb \begin{symbollist} } environment ensures that entries are
% %properly spaced.

% %\section*{Symbols}

% %Put general notes about symbol usage in text here.  Notice this text is
% %double-spaced, as required.

% %\begin{symbollist}
% 	%\item[$\mathbb{X}$] A blackboard bold $X$.  Neat.
% 	% Optional item argument makes the symbol/abbr
% 	%\item[$\mathcal{X}$] A caligraphic $X$.  Neat.
% 	%\item[$\mathfrak{X}$] A fraktur $X$.  Neat.
% 	%\item[$\mathbf{X}$] A boldface $X$.
% 	%\item[$\mathsf{X}$] A sans-serif $X$. Bad notation.
% 	%\item[$\mathrm{X}$] A roman $X$.
% %\end{symbollist}

% \section*{Abbreviations}

% %Long lines in the \texttt{symbollist} environment are single spaced, like in
% %the other front matter tables.

% \begin{symbollist}
% 	\item[DT] The frequency matrix Docs x Terms, $DT$:  Each row represents a document and each column represents a particular term. $DT(i,j)$ represents how many times term $j$ appears in document $i$.
% 	\item[DC] The frequency matrix Docs x Term Clusters, $DC$:  Each row represents a document and each column represents a particular term cluster. $DC(i,j)$ represents how many times words in term cluster $j$ appear in document $i$.

% \end{symbollist}


==> CHANGELOG <==
Version 0.4:
Removed features:
* parts. Does not comply with G-school style
* two-column signature page. Can only have up to six members.
* Duke logo
Bug fixes
* fixed double-spacing in List of Tables.

Version 0.3:
New features:
* "oldstyle" returns to the standard LaTeX report style for headings 
* "nobind" centers the text on the page (and it's now on by default in economy) 
Bug fixes
* Fixed dedication format and placement 
* Fixed small spelling errors in dissertation.tex (oops!)
* Fixed single-spacing in body when there are no frontmatter chapters

Version 0.25:
* Fixed bug in 'economy' option not playing nice with other options
* Tweaked section headers to be slightly smaller
* Make \raggedbottom the default page layout to avoid lots of underful vboxes
* ifpdf.sty no longer required
* Added fix_bookmarks.py hack to work-around missing features in hyperref

Version 0.2:
* Fixed warning during compliation from hyperref
* Automatic entry of PDF metadata from title and author fields.
* Citation hyperlinks working (but no more grouped cite support)
* Improved floatpage formatting.
* Support for longer titles, up to four lines

--------------------------------------------------
Version 0.1:
Released to a select audience.  Essentially functional.

